Cobol2Vec: Learning Representations of Cobol code

There has been a steadily growing interest in development of novel methods to learn a representation of a given input data and subsequently using them for several downstream tasks. The field of natural language processing has seen a significant improvement in different tasks by incorporating pre-trained embeddings into their pipelines. Recently, these methods have been applied to programming languages with a view to improve developer productivity. In this paper, we present an unsupervised learning approach to encode old mainframe languages into a fixed dimensional vector space. We use COBOL as our motivating example and create a corpus and demonstrate the efficacy of our approach in a code-retrieval task on our corpus.

==> tables/retrieval_results.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{p{.5\textwidth}|p{.6\textwidth}}
    \hline
    Query & Results \\
    \hline
    \hline
    
    \texttt{PERFORM VARYING SUB FROM INT BY INT UNTIL 
SUB $>$ RQDG-01-TOT-DRIVERS-CNT 
  IF LS-11-ORIG-DATE-LICS ( SUB ) NOT = SPACES 
  MOVE STR TO LS-MISC-CALCS-REQUEST-IND ( INT ) 
  ADD INT TO LS-MISC-CALC-COUNT  
  MOVE RQDG-01-TOT-DRIVERS-CNT TO SUB 
  END-IF 
END-PERFORM .} 

% PERFORM VARYING SUB1 FROM INT BY INT UNTIL \n SUB1 < INT OR TXT-FND \n IF SEG14-LIC-AG-TIN ( SUB1 : INT ) > SPACES \n SET TXT-FND TO TRUE \n MOVE SUB1 TO WS-FLD-LNGTH \n END-IF\n END-PERFORM .\\
& \texttt{PERFORM VARYING TBL-SUB FROM INT BY INT UNTIL \n TBL-SUB > NUM-OF-TERMS OR POLICY-TERM-FOUND \n IF WS-TERMDAYS ( TBL-SUB ) = WS-TERMDYS \n SET POLICY-TERM-FOUND TO TRUE \n MOVE WS-POLICY-TERM ( TBL-SUB ) \n TO RQDG-22-POLICY-TERM \n END-IF \n END-PERFORM .
2478,MOVE DATA-ID TO DATA-ID .,
MOVE WS-SPMK-IND TO RQDG-RA-SPMKTG-IND .} \\
& \texttt{PERFORM VARYING TBL-SUB FROM INT BY INT UNTIL \n TBL-SUB > NUM-OF-TERMS OR POLICY-TERM-FOUND \n IF WS-TERMDAYS ( TBL-SUB ) = WS-TERMDYS \n SET POLICY-TERM-FOUND TO TRUE \n MOVE WS-POLICY-TERM ( TBL-SUB ) \n TO RQDG-22-POLICY-TERM \n END-IF \n END-PERFORM .
2478,MOVE DATA-ID TO DATA-ID .,MOVE WS-SPMK-IND TO RQDG-RA-SPMKTG-IND .
}

    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

% \multirow{3}{*} 

% PERFORM VARYING SUB FROM INT BY INT UNTIL 
% SUB $>$ RQDG-01-TOT-DRIVERS-CNT 
%   IF LS-11-ORIG-DATE-LICS ( SUB ) NOT = SPACES 
%   MOVE STR TO LS-MISC-CALCS-REQUEST-IND ( INT ) 
%   ADD INT TO LS-MISC-CALC-COUNT  
%   MOVE RQDG-01-TOT-DRIVERS-CNT TO SUB 
%   END-IF 
% END-PERFORM .
